Black Swan: Abductive and Defeasible Video Reasoning in Unpredictable Events

The commonsense reasoning capabilities of vision-language models (VLMs), especially in abductive reasoning and defeasible reasoning, remain poorly understood. Most benchmarks focus on typical visual scenarios, making it difficult to discern whether model performance stems from keen perception and reasoning skills, or reliance on pure statistical recall. We argue that by focusing on atypical events in videos, clearer insights can be gained on the core capabilities of VLMs. Explaining and understanding such out-of-distribution events requires models to extend beyond basic pattern recognition and regurgitation of their prior knowledge. To this end, we introduce BlackSwanSuite, a benchmark for evaluating VLMs' ability to reason about unexpected events through abductive and defeasible tasks. Our tasks artificially limit the amount of visual information provided to models while questioning them about hidden unexpected events, or provide new visual information that could change an existing hypothesis about the event. We curate a comprehensive benchmark suite comprising over 3,800 MCQ, 4,900 generative and 6,700 yes/no questions, spanning 1,655 videos. After extensively evaluating various state-of-the-art VLMs, including GPT-4o and Gemini 1.5 Pro, as well as open-source VLMs such as LLaVA-Video, we find significant performance gaps of up to 32% from humans on these tasks. Our findings reveal key limitations in current VLMs, emphasizing the need for enhanced model architectures and training strategies. Our data and leaderboard is available at blackswan.cs.ubc.ca.

==> sections/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sections/3-definitions.tex <==
% Explaining surprising events requires models to go beyond pattern matching and have a deeper understanding of the world. A human-like understanding of the world can, in turn, improve VLMs' capabilities across the board, including video summarization and generation. 







% Furthermore, they can also---to a great extent---make predictions about future events or reason about incomplete information. For instance, observing two damaged cars at the middle of an intersection on a snowy day, we can hypothesize that this was caused by a weather related car accident. Humans are also naturally adept at updating beliefs and making inferences when presented with novel or contradictory information—a skill known as non-monotonic reasoning, where new evidence can invalidate prior conclusions.
% \cite{Shank1998TheEO} -- why its important
% This seemingly trivial human ability is still challenging for models due to the need for dynamic inference, where conclusions may need to shift with new or contradictory inputs. This ability to revise inferences on the fly is still an active area of research in AI and cognitive science
% the genre of surprising videos is extremely popular online, as they pique human curiosity and elicit reactions from users.  
%“Surprise” or “Unexpected” videos are the domain of videos that elicit a reaction from human viewers, as they often contain situations where something that is generally unlikely to happen ends up happening. Such videos are extremely popular, and are often seen on social media platforms because they pique human curiosity. More importantly,
% Humans can understand what led to a surprising outcome. %, and understand sudden changes in the video scene. 

% without even observing a surprising event happening (e.g. a car accident as it happens), but only observing the outcome of the event (two damaged cars at the middle of an intersection), humans can estimate possible means that led to that outcome. What may seem like an easy task to humans, is an extremely challenging task for AI models.
% As such, models must be capable of (1) predicting many possibilities of what could happen in a scene, (2) deriving a reasonable path to arrive at the surprising outcome, and (3) gaining capability to understand and reason about situations that are out-of-domain. In general, it requires the model to understand the mechanisms of the world, as well as to understand feelings and reactions from humans that appear in such videos.
% (PARA2: building a world model and achieving general intelligence. (1) and (2) tells apart the ordinary from the surprising -- it is a result of the world model. This has two benefits, - this is a good test for the world model, and - humans are interested in these kinds of vidoes, but why? Allows them to learn beyond the mode of the distb. Sora is an evidence of the (lack of) a good world model)

% (old Para 2 comes here)
% Furthermore, research in this direction can guide future works in video generation, where current video models change in situations where there a sudden state change is required (eg. the Sora video of blowing out candles). Building capabilities to understand such videos can also reduce hallucination in video captioning.

% Several recent works in the VLM literature extend image understanding and reasoning capabilities to multi-frame videos. These works 
% they struggle in cases where there is an element of surprise. (Look for citations; alternatively, models are good at the mode of the dist but not in the rare cases, surprises are cases which are rare, never seen happening.)



 

==> sections/intro-old.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=1.0\linewidth]{figures/VARmain.pdf}
   \caption{\textbf{\bench{}}. Our benchmark involves three tasks, \taskOne{}, \taskTwo{} and \taskThree, briefly described above.}
   \label{fig:tasks}
\end{figure*}

% 1) VLMs can do basic reasoning about the expected event.
%Vision-language models (VLMs) are becoming increasingly capable of reasoning about the world thanks to their exposure to vast amounts of images or videos, and the reasoning capabilities of their underlying large language models (LLMs). 

% Recent multi-frame video-language models such as VILA \cite{lin2023vila}, Video-LLaMA \cite{cheng2024videollama2}, and LLaVA-Video \cite{zhang2024llavavideo} show promising results in tasks such as video captioning and question answering.
% % (2) they struggle with unexpected events because they simply do pattern recognition, rather than have a world model.
% Nonetheless, 
% %while these models may be able to understand the events in the video or even predict the following events, based on patterns in their vast training data, 
% it remains unclear to what extent they are capable of commonsense reasoning over unexpected and surprising events. The human ability to effectively recognize, rationalize, learn from, and respond to rare and surprising events is underpinned by two reasoning capabilities, 
% %achieve a robust understanding of the world through flexible world models that allow them to make sense of surprising events and adapt to sudden state changes in dynamic environments. A key part of this ability lies in 
% \emph{abductive reasoning} \cite{Hessel2022TheAO,Liang2022VisualAR,Zhao2022VideoABCAR}---drawing the most likely explanation from limited observations---and \emph{defeasible reasoning} \cite{han-etal-2023-reading}, which makes rationally compelling initial inferences and later revises them in light of new evidence. For example, upon observing two damaged cars in an intersection on a snowy day, a human driver may, through abductive reasoning, hypothesize that the cause is slippery road surface. However, if the driver later learns about a car manufacturer recalling its products due to brake faults in low temperature, through defeasible reasoning they can modify the initial hypothesis to faulty brakes and possibly exercise  extra caution when near such cars. 
% %and (2) through defeasible reasoning, revise their initial belief that driving to work today would be easy. 


Recent multi-frame video-language models such as VILA \cite{lin2023vila}, Video-LLaMA \cite{cheng2024videollama2}, and LLaVA-Video \cite{zhang2024llavavideo} show promising results in tasks such as video captioning and question answering. Nonetheless, it remains unclear to what extent they are capable of reasoning over unexpected events. 


The human ability to effectively recognize, rationalize, and respond to unexpected events is underpinned by two types of reasoning, \emph{abductive reasoning} \cite{Hessel2022TheAO,Liang2022VisualAR,Zhao2022VideoABCAR} and \emph{defeasible reasoning} \cite{han-etal-2023-reading}. 

%For example, a human may observe two damaged cars in an intersection on a snowy day, and hypothesize that an accident was caused by the slippery road surface.

However, if the driver later learns about a car manufacturer recalling its products due to brake faults in low temperature, through defeasible reasoning they can modify the initial hypothesis to faulty brakes and possibly exercise  extra caution when near such cars. 
%and (2) through defeasible reasoning, revise their initial belief that driving to work today would be easy. 

%achieve a robust understanding of the world through flexible world models that allow them to make sense of surprising events and adapt to sudden state changes in dynamic environments. A key part of this ability lies in 
%while these models may be able to understand the events in the video or even predict the following events, based on patterns in their vast training data, 



Unexpected events pose a unique challenge in machine learning. As expectations are built on frequency, unexpected events by definition are rare in life and scarce in training data, and may be overlooked by stochastic gradient descent \cite{role-of-memorization-2017,pmlr-v97-rahaman19a,Dimitris2019}.
%As a result, they tend to be overlooked by stochastic gradient descent, which prioritizes learning simple patterns over complex patterns \cite{role-of-memorization-2017,pmlr-v97-rahaman19a,Dimitris2019}. 
Overfitting to frequent events has been widely reported, such as video models classifying all events happening on soccer fields as \emph{playing soccer}~\cite{zhang2024dont,Li_2023_ICCV,NEURIPS2023_aef34c77,bae2024devias}. If AI models are to function as autonomous decision makers ({\em e.g.}, in self-driving vehicles \cite{OKelly2018,Wang2021AdvSim}), reasoning about unexpected events abductively and defeasibly would be critical to their safety and real-world utility.

% (3) the world model helps humans with abductive and defeasible reasoning, with the car accident example.
% In contrast, 
%a weather-related accident, quickly adapting their reasoning to account for contextual clues. Furthermore, such an observation may influence their driving style, and awareness of their surroundings. 

% Such reasoning processes are fundamental to human adaptability.  As discussed earlier, VLMs trained mainly on frequent events  may not function well when normal expectations are violated. 

%, which tend to rely heavily on familiar data patterns without a robust underlying world model.

% (4) world modeling is important for summarization and generation: plot twists in movies, sudden state change in Sora video. 

% World models capable of understanding surprising events could enhance VLMs’ performance across a range of applications, from summarizing videos with complex plot twists to generating realistic scenes that include sudden changes \sahi{cite SORA}. Furthermore, 


% (5) So, there is a need to test this capability, and we propose \bench{}. (6) define contributions}

In this paper, we present the \textbf{\bench{}} benchmark, with a range of tasks that require nuanced perception, comprehension, and reasoning abilities. We focus on leveraging the visual information provided in videos of expectation-violating events, including but not limited to surprises, accidents, pranks and other uncommon situations. Such videos are ideal for evaluating abductive and defeasible reasoning capabilities of models, as these events occur scarcely, if ever, in the training data, and regurgitation of seen data arguably would be  insufficient. Our benchmark consists of three overarching tasks (Fig \ref{fig:tasks}), named \taskOne, \taskTwo\, and \taskThree, involving 15,469 sub-tasks, with both generative and discriminative variants. 

We evaluate leading closed-source and open-source video and multi-frame VLMs on our tasks. Results indicate that the best models lag behind humans by up to 25\% on MCQ and 32\% on Y/N variants.
%, indicating a significant potential for improvements on our reasoning tasks. 
By highlighting the limitations of current VLMs on reasoning tasks, \bench{} can drive the development of future models with stronger reasoning abilities.

% We pose \bench{} as an initial tool to evaluate models that, in the near future, promise to be perceptually faithful, factual, logical as well as have innately human capabilities (e.g., understanding humor and surprise, which would benefit human-computer interactions more broadly). Ultimately, we hope that it will drive future research toward developing VLMs with deeper reasoning capabilities, enhancing their performance across a wide range of vision-language tasks. \abl{can shorten this paragraph, or move part of to conclusions.}
% \vered{Alternative suggestion: move the last sentence from the previous paragraph ``we evaluate leading...'' and add ``By highlighting the limitations of current VLMs in reasoning [...] \bench{} can drive the development of future models with stronger reasoning abilities.'' (need to better phrase).} 

% \vered{I'm not a fan of the ``our contributions'' paragraph personally. I would prefer to just continue the previous paragraph describing the evaluation and the main results, and then ending with a sentence about how this benchmark can drive future research for improving VLMs in general.}




% \adi{We should work on the flow of this introduction. The flow in my mind: (1) VLMs can do basic reasoning about expected event. (2) they struggle with unexpected events because they simply do pattern recognition, rather than have a world model. (3) the world model helps humans with abductive and defeasible reasoning, with the car accident example. (4) world modeling is important for summarization and generation: plot twists in movies, sudden state change in Sora video. (5) So, there is a need to test this capability, and we propose \bench{}. (6) define contributions}




% Vision-language models (VLMs) are becoming increas-
% ingly capable of reasoning about the world thanks to their
% exposure to vast amounts of images or videos, and the rea- soning capabilities of their underlying large language mod- els (LLMs). Recent multi-frame video models such as 038
% [9, 24, 25] show promising results in tasks such as video captioning and question answering. 040
% Nonetheless, while these models may be able to under- stand the events in the video or even predict the following events, based on patterns in their vast training data, it re- mains unclear to what extent they are capable of making predictions on unexpected events. 045
% In contrast, humans achieve a robust understanding of the world through flexible world models that allow them to make sense of surprising events and adapt to sudden state changes in dynamic environments. A key part of this ability lies in abductive reasoning—drawing the most likely expla- nation from limited observations—and defeasible reason- ing, where initial conclusions are revised in light of new or conflicting evidence. For example, upon observing two damaged cars in an intersection on a snowy day, humans naturally hypothesize a weather-related accident, quickly adapting their reasoning to account for contextual clues. This reasoning process is fundamental to human adaptabil- ity, yet it remains an ongoing challenge for VLMs, which tend to rely heavily on familiar data patterns without a ro- bust underlying world model. 060
% World models capable of understanding surprising events could enhance VLMs’ performance across a range of applications, from summarizing videos with complex plot twists to generating realistic scenes that include sud- den changes [cite SORA]−SR 065
% In this paper, we present the BlackSwanSuite bench- mark, with a range of tasks that require understanding and reasoning about videos with unexpected events. Our bench- mark consists of [X]−V S tasks, available in both genera- tive and discriminative variants. We evaluate leading Video LMs, Multi-frame Image VLMs, and LLMs on our gener- ative and discriminative tasks. We hope that BlackSwan- 072
% Suite will drive future research toward developing VLMs with deeper reasoning capabilities, ultimately enhancing their performance across a wide range of vision-language 

==> tables/generative-res.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{lrrrrrrrr}
\toprule
\textbf{Model} & \textbf{BLEU} & \textbf{ROUGE-L} & \textbf{CLIPScore} & \textbf{LLM Match} & \multicolumn{1}{r}{\textbf{Human - C}} & \multicolumn{1}{r}{\textbf{Human - T}} & \multicolumn{1}{r}{\textbf{Human - D}} & \multicolumn{1}{r}{\textbf{Human - V}} \\

\midrule
\rowcolor{orange!30} \multicolumn{9}{c}{\textbf{\taskOne{}}} \\
\midrule
GPT-4o & 0.0070 & 0.2710 & 0.769 & 1.58 & \multicolumn{1}{r}{3.72} & \multicolumn{1}{r}{3.62} & \multicolumn{1}{r}{3.81} & \multicolumn{1}{r}{0.91} \\
Gemini 1.5 Pro & 0.0126 & 0.2803 & 0.779 & 1.60 &  &  &  &  \\
VideoChat 2 & 0.0049 & 0.2580 & 0.708 & 1.64 & \multicolumn{1}{r}{3.15} & \multicolumn{1}{r}{3} & \multicolumn{1}{r}{3.1} & \multicolumn{1}{r}{0.8} \\
VideoLlama2 & 0.0067 & 0.2520 & 0.776 & 1.44 & \multicolumn{1}{r}{3.25} & \multicolumn{1}{r}{2.7} & \multicolumn{1}{r}{3.15} & \multicolumn{1}{r}{0.85} \\
VILA & 0.0080 & 0.1877 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  \\
LLaVA-Video & 0.0049 & 0.2050 & 0.645 & 1.55 & \multicolumn{1}{r}{3.73} & \multicolumn{1}{r}{3.73} & \multicolumn{1}{r}{3.96} & \multicolumn{1}{r}{0.81} \\
LLaVA-Video 72B & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  \\
Human & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  \\

\midrule
\rowcolor{orange!30} \multicolumn{9}{c}{\textbf{\taskTwo{}}} \\
\midrule
GPT-4o & 0.0080 & 0.2606 & 0.777 & 3.404 & \multicolumn{1}{r}{3.25} & \multicolumn{1}{r}{3} & \multicolumn{1}{r}{3.15} & \multicolumn{1}{r}{0.7} \\
Gemini 1.5 Pro & 0.0112 & 0.2414 & 0.733 & 3.400 &  &  &  &  \\
VideoChat 2 & 0.0100 & 0.2604 & 0.680 & 3.070 &  &  &  &  \\
VideoLlama2 & 0.0011 & 0.1542 & 0.614 & 2.728 &  &  &  &  \\
VILA & 0.0083 & 0.1659 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  \\
LLaVA-Video & 0.0061 & 0.2428 & 0.585 & 3.179 & \multicolumn{1}{r}{3.35} & \multicolumn{1}{r}{3.3} & \multicolumn{1}{r}{3} & \multicolumn{1}{r}{0.75} \\
LLaVA-Video 72B & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  \\
Human & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  \\

\midrule
\rowcolor{orange!30} \multicolumn{9}{c}{\textbf{\taskThree{}}} \\
\midrule
GPT-4o & 0.0090 & 0.2340 & 0.647 & 3.35 &  &  &  &  \\
Gemini 1.5 Pro & 0.0043 & 0.1190 & 0.504 & 3.35 &  &  &  &  \\
VideoChat 2 & 0.0070 & 0.2090 & 0.612 & 2.66 &  &  &  &  \\
VideoLlama2 & 0.0052 & 0.1730 & 0.658 & 2.57 &  &  &  &  \\
VILA & 0.0060 & 0.1530 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  \\
LLaVA-Video & 0.0081 & 0.2050 & 0.573 & 2.691 &  &  &  &  \\
LLaVA-Video 72B & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  \\
Human & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  & \\
\bottomrule
\end{tabular}
  \caption{\textbf{Results for Generative}}
  \label{tab:genresults}
\end{table*}

==> tables/humaneval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

%\setlength{\tabcolsep}{8pt}

\begin{table*}[t]
\centering
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{4}{c}{\cellcolor[HTML]{F4EDE5}\textbf{Forecaster}} & \multicolumn{4}{c}{\cellcolor[HTML]{E3F6E3}\textbf{Detective}} & \multicolumn{4}{c}{\cellcolor[HTML]{E1EAF6}\textbf{Reporter}} \\
{} & {\textbf{C}} & {\textbf{T}} & {\textbf{D}} & {\textbf{V}} & {\textbf{C}} & {\textbf{T}} & {\textbf{D}} & {\textbf{V}} & {\textbf{C}} & {\textbf{T}} & {\textbf{D}} & {\textbf{V}} \\
\midrule
\rowcolor{gray!20} \multicolumn{13}{c}{\textbf{Closed Source}} \\
GPT-4o & \textbf{3.72} & \textbf{3.62} & \textbf{3.81} & \textbf{0.91} & 3.41 & 3.28 & 3.53 & 0.78 & 4.10 & 3.50 & 3.70 & 0.90 \\
Gemini 1.5 Pro & - & - & - & - & - & - & - & - & - & - & - & - \\
\rowcolor{gray!20} \multicolumn{13}{c}{\textbf{Open Source}} \\
VideoChat 2 & 3.57 & 3.38 & 3.43 & 0.86 & 3.60 & 2.90 & 3.20 & 0.75 & - & - & - & - \\
VideoLlama2 & 3.05 & 2.80 & 3.50 & 0.80 & - & - & - & - & - & - & - & - \\
VILA & - & - & - & - & - & - & - & - & - & - & - & - \\
Llava-Video & 3.41 & 3.53 & 3.75 & 0.78 & 2.70 & 2.35 & 2.70 & 0.55 & - & - & - & - \\
\rowcolor{gray!20} \multicolumn{13}{c}{\textbf{Human}} \\
Human & 2.89 & 3.04 & 3.00 & 0.71 & \textbf{4.11} & \textbf{3.89} & \textbf{3.90} & \textbf{0.79} & \textbf{4.40} & \textbf{3.85} & \textbf{3.90} & \textbf{0.95} \\
\bottomrule
\end{tabular}
\caption{\textbf{Human Eval Results:} We evaluate all models on 30 randomly sampled videos from our dataset, across all three tasks, and ask humans to rate on Correctness (\textbf{C}), Depth and Thoughtfulness (\textbf{T}), Level of Detail (\textbf{D}) and Visual Entailment (\textbf{V}). All scores are normalized to 0-1 range, and higher is better.}
\label{tab:humaneval}
\end{table*}

==> tables/mainresults.tex <==
\begin{table*}[ht]
  \centering
  \begin{tabular}{lccc}
    \toprule
    \textbf{Model} & \textbf{Task 1} & \textbf{Task 2} & \textbf{Overall} \\
     \# Questions:       & 1190 & 160 & 1350 \\ 
    \midrule
    \rowcolor{gray!20} \multicolumn{4}{c}{\textbf{Video LM}} \\
    VideoLlama 2 (7b) & 0.447 & 0.55 & 0.46 \\
    Llava-Video (7b) & 0.47 & 0.68 & 0.49 \\
    \midrule
    \rowcolor{gray!20} \multicolumn{4}{c}{\textbf{Multi-frame VLLM}} \\
    GPT-4V & 0.45 & 0.75 &  \\
    VILA (7b) & 0.5013 & 0.5635 &  \\
    \midrule
    \rowcolor{gray!20} \multicolumn{4}{c}{\textbf{LLM with Video Caption}} \\
    Llama 2 (7b) &  &  &  \\
    GPT-4o &  &  &  \\
    \midrule
    \rowcolor{gray!20} \multicolumn{4}{c}{\textbf{Human Performance}} \\
    Human Expert & \textbf{0.73} & \textbf{0.85} &  \\
    \bottomrule
  \end{tabular}
  %\vspace{-0.2cm}
  \caption{\textbf{MCQ Task Results:} 
  }
  \label{tab:userstudy1}
  %\vspace{-0.2cm}
\end{table*}

==> tables/subtasks.tex <==


\begin{table*}[t]
\centering
\begin{tabular}{|c|c|p{0.3\textwidth}|}
\hline
\textbf{Task} & \textbf{Task Variant} & \textbf{Description / Explanation} \\ \hline
\multirow{2}{*}{Task 1: Predict the Future} 
& Gen: Generate free-text answer & Predict "What happens next?" based on pre-event context. \\ \cline{2-3} 
& --- & Model infers future events based on setup context. \\ \hline
\multirow{3}{*}{Task 2: Reconstruct the Missing Event} 
& Gen: Generate free-text answer & Infer "What happened in the middle?" based on surrounding context. \\ \cline{2-3}
& MCQ: Multiple Choice & Select the correct middle event from 3 options. \\ \cline{2-3}
& Def: Defeasibility Assessment & Validate a hypothesis about the middle event. \\ \hline
\multirow{3}{*}{Task 3: Explain the Sequence} 
& Gen: Generate free-text explanation & Describe the entire video sequence. \\ \cline{2-3}
& MCQ: Multiple Choice & Select the correct description of the entire video. \\ \cline{2-3}
& Def: Defeasibility Assessment & Evaluate a hypothesis about the events after seeing the full video. \\ \hline
\end{tabular}
\caption{Task variants and descriptions for evaluating video reasoning.}
\end{table*}


==> tables/task1-old.tex <==
\setlength{\tabcolsep}{2pt}

\begin{table}[t]
  \centering
  \small
  \begin{tabular}{lrrrrrr}
    \toprule
    \textbf{Model} & \multicolumn{5}{c}{\textbf{Generative}} & \textbf{MCQ} \\ \cmidrule{2-7}
     \multirow{2}{*}{Metrics \xrightarrow} & BLEU & \multirow{2}{*}{ROUGE} & CLIP & GPT & Human & Acc \\ 
     & ($\times 10^{-3}$) &  & Score & Score & Rating &  (\%) \\ 
    \midrule
    \rowcolor{gray!20} \multicolumn{7}{c}{\textbf{Closed Source}} \\
    GPT-4o & X & X & X & X & X & - \\
    Gemini-1.5 Pro & X & X & X & X & X & - \\
    \rowcolor{gray!20} \multicolumn{7}{c}{\textbf{Open Source}} \\
    VideoChat2  & 4.91 & 0.220 & 0.707 & X & X & - \\
    % VideoChatGPT & X & X & X & X & X & - \\
    VILA (7B) & X & X & X & X & X & - \\
    VILA (34B) & X & X & X & X & X & - \\
    VideoLlama2 & 6.6 & 0.252 & 0.776 & X & X & - \\
    Qwen VL Max & X & X & X & X & X & - \\
    LLaVAVideo (7B)  & 4.98 & 0.205 & 0.645 & X & X & - \\
    LLaVAVideo (70B) & X & X & X & X & X & - \\
    % \rowcolor{gray!20} \multicolumn{7}{c}{\textbf{Open Source LLM w/ Summarization}} \\
    % Llama 3.2 w/ LLaVAVideo & X & X & X & X & X & - \\
    % Llama 3.2 w/ Human & X & X & X & X & X & - \\
    \rowcolor{gray!20} \multicolumn{7}{c}{\textbf{Human Performance}} \\
    Human Expert & X & X & X & X & X & - \\
    \bottomrule
  \end{tabular}
  %\vspace{-0.2cm}
  \caption{\textbf{Results for Task 1: What happens next?} ...}
  \label{tab:task1}
  %\vspace{-0.2cm}
\end{table}


==> tables/task1.tex <==
%\setlength{\tabcolsep}{2pt}

\begin{table}[t]
  \centering
  \begin{tabular}{lcc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c}{\textbf{Generative}} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{CLIP}} & \multicolumn{1}{c}{\textbf{LLM-M}} \\
    \midrule
    \rowcolor{gray!20} \multicolumn{3}{c}{\textbf{Closed Source}} \\
    GPT-4o & 0.77 & 1.58 \\
    Gemini 1.5 Pro & \textbf{0.78} & 1.60 \\
    \rowcolor{gray!20} \multicolumn{3}{c}{\textbf{Open Source}} \\
    VideoChat2 & 0.71 & \textbf{1.64} \\
    VideoLLaMA 2 & \textbf{0.78} & 1.44 \\
    VILA-1.5 & 0.66 & 1.49 \\
    LLaVA-Video & 0.64 & 1.55 \\
    \rowcolor{gray!20} \multicolumn{3}{c}{\textbf{Human}} \\
    Human & 0.76 & \multicolumn{1}{l}{-} \\
    \bottomrule
  \end{tabular}
  %\vspace{-0.2cm}
  \caption{\textbf{Results on \taskOne.}}
  \label{tab:task1}
  %\vspace{-0.2cm}
\end{table}


==> tables/task2-old.tex <==
% \newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
\setlength{\tabcolsep}{1pt}


\begin{table}[t]
  \centering
  \small
  \begin{tabular}{lrrrrrrr}
    \toprule
    \textbf{Model} & \multicolumn{5}{c}{\textbf{Generative}} & \textbf{MCQ} & \textbf{Yes/No} \\ \cmidrule{2-8}
     \multirow{2}{*}{Metrics \xrightarrow} & BLEU & \multirow{2}{*}{ROUGE} & CLIP & GPT & Human & Acc & Acc \\ 
     & {\tiny ($\times 10^{-3}$)} &  & Score & Score & Rating &  (\%) & (\%) \\ 
    \midrule
    \rowcolor{gray!20} \multicolumn{8}{c}{\textbf{Closed Source}} \\
    GPT-4o & X & X & X & X & X & 67.1 \\
    Gemini-1.5 Pro & X & X & X & X & X & 52.3 \\
    \rowcolor{gray!20} \multicolumn{8}{c}{\textbf{Open Source}} \\
    VideoChat2 & 4.36 & 0.221 & 0.697 & X & X & 29.9 & 63.0 \\
    % VideoChatGPT  & X & X & X & X & X & X \\
    VILA (8B)  & X & X & X & X & X & %50.13 \\
    50.1 \\
    VILA (34B)  & X & X & X & X & X & X \\
    VideoLlama 2  & %0.00063 
    0.63 & 0.134 & 0.693 & X & X & 45.7 \\
    Qwen VL Max  & X & X & X & X & X & X \\
    LLaVAVideo (7B) & %0.00269 
    2.69 & 0.183 & 0.622 & X & X & 55.9 & 59.3\\
    LLaVAVideo (70B) & X & X & X & X & X & X \\
    % \rowcolor{gray!20} \multicolumn{7}{c}{\textbf{Open Source LLM w/ Summarization}} \\
    % Llama 3.2 w/ LLaVAVideo & X & X & X & X & X & X \\
    % Llama 3.2 w/ Human & X & X & X & X & X & X \\
    \rowcolor{gray!20} \multicolumn{8}{c}{\textbf{Human Performance}} \\
    Human Expert & X & X & X & X & X & 90.0 \\
    \bottomrule
  \end{tabular}
  %\vspace{-0.2cm}
  \caption{\textbf{Results for Task 2: What could have happened in the middle?} ...}
  \label{tab:task2}
  %\vspace{-0.2cm}
\end{table}

==> tables/task2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c}{\textbf{Generative}} & \multicolumn{1}{c}{\textbf{MCQ}} & \multicolumn{1}{c}{\textbf{Y/N}} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{CLIP}} & \multicolumn{1}{c}{\textbf{LLM-M}} & \multicolumn{1}{c}{\textbf{(\%)}} & \multicolumn{1}{c}{\textbf{(\%)}} \\
\midrule
\rowcolor{gray!20} \multicolumn{5}{c}{\textbf{Closed Source}} \\
GPT-4o & \textbf{0.78} & \textbf{3.40} & 67.1 & 62.4 \\
Gemini 1.5 Pro & 0.73 & \textbf{3.40} & 52.3 & 63.2 \\
\rowcolor{gray!20} \multicolumn{5}{c}{\textbf{Open Source}} \\
VideoChat2 & 0.68 & 3.07 & 29.9 & 63.0 \\
VideoLLaMA 2 & 0.61 & 2.73 & 45.7 & 57.7 \\
VILA-1.5 & 0.50 & 3.17 & 51.8 & 57.6 \\
LLaVA-Video & 0.58 & 3.18 & 55.9 & 59.3 \\
\rowcolor{gray!20} \multicolumn{5}{c}{\textbf{Human}} \\
Human & 0.77 & \multicolumn{1}{l}{-} & \textbf{90.0} & \multicolumn{1}{l}{-} \\
\bottomrule
\end{tabular}
\caption{\textbf{Results on \taskTwo.}}
\label{tab:task2}
\end{table}

==> tables/task3-old.tex <==
% \begin{table*}[ht]
%   \centering
%   \begin{tabular}{lcccccc}
%     \toprule
%     \textbf{Model} & \multicolumn{5}{c}{\textbf{Generative}} & \textbf{MCQ} \\
%      Metrics \xrightarrow & BLEU & ROUGE & CLIP Score & GPT-score & Human Rating & Acc (\%) \\ 
\setlength{\tabcolsep}{1pt}

\begin{table}[t]
  \centering
  \small
  \begin{tabular}{lrrrrrrr}
    \toprule
    \textbf{Model} & \multicolumn{5}{c}{\textbf{Generative}} & \textbf{MCQ} & \textbf{Yes/No} \\ \cmidrule{2-8}
     \multirow{2}{*}{Metrics \xrightarrow} & BLEU & ROUGE & CLIP & GPT & Human & Acc & Acc \\ 
     & {\tiny ($\times 10^{-3}$)} & {\tiny ($\times 10^{-2}$)} & Score & Score & Rating &  (\%) &  (\%) \\ 
    \midrule
    \rowcolor{gray!20} \multicolumn{8}{c}{\textbf{Closed Source}} \\
    GPT-4o  & X & X & X & X & X & 73.8 \\
    Gemini-1.5 Pro & X & X & X & X & X & 62.7 \\
    \rowcolor{gray!20} \multicolumn{8}{c}{\textbf{Open Source}} \\
    VideoChat2 & 1.56 & 8.56 & 0.499 & X & X & 51.6 & 44.3 \\
    % VideoChatGPT  & X & X & X & X & X & X \\
    VILA (8B) & X & X & X & X & X & % 56.35\% \\
    56.4 \\
    VILA (34B) & X & X & X & X & X & X \\
    VideoLlama 2 & 0.78 & 6.8 & 0.557 & X & X & 53.7 \\
    Qwen VL Max  & X & X & X & X & X & X \\
    LLaVAVideo (7B)  & 1.15 & 8.28 & 0.451 & X & X & 69.6 & 55.1\\
    LLaVAVideo (70B) & X & X & X & X & X & X \\
    % \rowcolor{gray!20} \multicolumn{7}{c}{\textbf{Open Source LLM w/ Summarization}} \\
    % Llama 3.2 w/ LlavaVideo & X & X & X & X & X & X \\
    % Llama 3.2 w/ Human  & X & X & X & X & X & X \\
    \rowcolor{gray!20} \multicolumn{8}{c}{\textbf{Human Performance}} \\
    Human Expert & X & X & X & X & X & 95.3 \\
    \bottomrule
  \end{tabular}
  %\vspace{-0.2cm}
  \caption{\textbf{Results for Task 3: Explain what happened.} ...}
  \label{tab:task3}
  %\vspace{-0.2cm}
\end{table}

==> tables/task3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c}{\textbf{Generative}} & \multicolumn{1}{c}{\textbf{MCQ}} & \multicolumn{1}{c}{\textbf{Y/N}} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{CLIP}} & \multicolumn{1}{c}{\textbf{LLM-M}} & \multicolumn{1}{c}{\textbf{(\%)}} & \multicolumn{1}{c}{\textbf{(\%)}} \\
\midrule
\rowcolor{gray!20} \multicolumn{5}{c}{\textbf{Closed Source}} \\
GPT-4o & 0.65 & 3.35 & 73.8 & 60.1 \\
Gemini 1.5 Pro & 0.50 & 3.35 & 62.7 & 52.9 \\
\rowcolor{gray!20} \multicolumn{5}{c}{\textbf{Open Source}} \\
VideoChat2 & 0.61 & 2.66 & 51.6 & 44.3 \\
VideoLLaMA 2 & 0.66 & 2.57 & 53.2 & 54.1 \\
VILA-1.5 & 0.40 & 2.84 & 54.3 & 50.6 \\
LLaVA-Video & 0.57 & 2.69 & 69.6 & 55.1 \\
\rowcolor{gray!20} \multicolumn{5}{c}{\textbf{Human}} \\
Human & \textbf{0.75} & \multicolumn{1}{l}{-} & \textbf{95.3} & \multicolumn{1}{l}{-}\\
\bottomrule
\end{tabular}
\caption{\textbf{Results on \taskThree.} }
\label{tab:task3}
\end{table}

==> tables/traditionalmetrics.tex <==
% \setlength{\tabcolsep}{2pt}
% \begin{table}[ht]
%   \centering
%   \small % Reduce font size for compactness
%   \begin{tabular}{lcccccc}
%     \toprule
%     \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{\taskOne}} & \multicolumn{2}{c}{\textbf{\taskTwo}} & \multicolumn{2}{c}{\textbf{\taskThree}} \\
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%     & \textbf{BLEU} & \textbf{ROUGE} & \textbf{BLEU} & \textbf{ROUGE} & \textbf{BLEU} & \textbf{ROUGE} \\
%     \midrule
%     % \rowcolor{gray!20} \multicolumn{7}{c}{\textbf{Closed Source}} \\
%     GPT-4o & 0.77 & 1.64 & 0.79 & 1.62 & 0.76 & 1.65 \\
%     Gemini 1.5 Pro & \textbf{\underline{0.78}} & 1.61 & 0.77 & 1.60 & 0.75 & 1.63 \\
%     \rowcolor{gray!20} \multicolumn{7}{c}{\textbf{Open Source}} \\
%     VideoChat2 & 0.71 & \underline{1.66} & 0.70 & 1.65 & 0.72 & 1.67 \\
%     VideoLLaMA 2 & \textbf{\underline{0.78}} & 1.45 & 0.76 & 1.44 & 0.74 & 1.46 \\
%     VILA-1.5 & 0.66 & 1.50 & 0.65 & 1.48 & 0.67 & 1.51 \\
%     LLaVA-V-7B & 0.64 & 1.57 & 0.58 & \underline{1.70} & 0.57 & \underline{2.36} \\
%       LLaVA-V-72B & \underline{0.69} & \underline{1.67} & \underline{0.60} & 1.68 & \underline{0.59} & 2.15 \\
%     \rowcolor{gray!20} \multicolumn{7}{c}{\textbf{Human}} \\
%     Human & \textbf{0.78} & \textbf{1.98} & \textbf{0.77} & \textbf{1.92} & \textbf{0.76} & \textbf{3.23} \\
%     \bottomrule
%   \end{tabular}
%   %\vspace{-0.2cm}
%   \caption{\textbf{Results on Gen variants with 72B version on 10\% of data.} Metrics are grouped by tasks, each with CLIP and LLM-M scores.}
%   \label{tab:traditionalmetri}
%   %\vspace{-0.2cm}
% \end{table}

